Investigating how ReLU-networks encode symmetries

Many data symmetries can be described in terms of group equivariance and the most common way of encoding group equivariances in neural networks is by building linear layers that are group equivariant. In this work we investigate whether equivariance of a network implies that all layers are equivariant. On the theoretical side we find cases where equivariance implies layerwise equivariance, but also demonstrate that this is not the case generally. Nevertheless, we conjecture that CNNs that are trained to be equivariant will exhibit layerwise equivariance and explain how this conjecture is a weaker version of the recent permutation conjecture by Entezari et al. [2022]. We perform quantitative experiments with VGG-nets on CIFAR10 and qualitative experiments with ResNets on ImageNet to illustrate and support our theoretical findings. These experiments are not only of interest for understanding how group equivariance is encoded in ReLU-networks, but they also give a new perspective on Entezari et al.'s permutation conjecture as we find that it is typically easier to merge a network with a group-transformed version of itself than merging two different networks.

==> gammal-teori.tex <==
\section{More formal things}
We begin by giving two standard definitions.
\begin{definition}
    Given a group $G$ and a set $X$, a \emph{group action} $\alpha$ of $G$ on $X$ is a function 
    \[
        \alpha : G\times X\to X
    \]
    such that for the identity element $i$ of $G$ and any $x\in X$ we have
    \begin{equation}
        \alpha(i, x) = x.
    \end{equation}
    and for any two $g, h\in G$ and any $x\in X$ we have
    \begin{equation}
        \alpha(hg, x) = \alpha(h, \alpha(g, x)).
    \end{equation}
\end{definition}

\begin{definition}
    Given a group $G$ and two sets $X$ and $Y$ with group actions $\alpha_X$ and $\alpha_Y$ respectively,
    a function $\phi: X\to Y$ is said to be \emph{($G$-)equivariant} with respect to 
    $\alpha_X$ and $\alpha_Y$ if
    for every $g\in G$ and $x\in X$
    \begin{equation}
        \phi(\alpha_X(g, x)) = \alpha_Y(g, \phi(x)).
    \end{equation}
\end{definition} 

\begin{lemma}
    Given a group $G$ and an invertible function $\phi: X\to Y$.
    \begin{enumerate}
        \item 
        If there is a group action $\alpha_X$ on $X$, then we can define a group action
        $\alpha_Y$ on $Y$ by
        \[
            \alpha_Y(g, y) = \phi(\alpha_X(g, \phi^{-1}(y)))
        \]
        and $\phi$ is equivariant with respect to this group action.
        \item
        Similarly, if there is a group action $\alpha_Y$ on $Y$, then we can define a group action
        $\alpha_X$ on $X$ by
        \[
            \alpha_X(g, x) = \phi^{-1}(\alpha_Y(g, \phi(x)))
        \]
        and $\phi$ is equivariant with respect to this group action.
    \end{enumerate}
\end{lemma} 
\begin{proof}
    We prove 1., the proof of 2. is analogous.
    $\alpha_Y$ is a group action as
    \[
        \alpha_Y(i, y) = \phi(\alpha_X(i, \phi^{-1}(y))) = \phi(\phi^{-1}(y)) = y
    \]
    and 
    \[
    \begin{split}
        \alpha_Y(hg, y) &= \phi(\alpha_X(hg, \phi^{-1}(y))) \\
        &= \phi(\alpha_X(h, \alpha_X(g, \phi^{-1}(y)))) \\
        &= \phi(\alpha_X(h, \phi^{-1}\circ\phi(\alpha_X(g, \phi^{-1}(y))))) \\
        &= \alpha_Y(h, \phi(\alpha_X(g, \phi^{-1}(y)))) \\
        &= \alpha_Y(h, \alpha_Y(g, y)).
    \end{split}
    \]
    $\phi$ is equivariant w.r.t. to $\alpha_X$ and $\alpha_Y$ by definition of $\alpha_Y$:
    \[
        \phi(\alpha_X(g, x)) = \phi(\alpha_X(g, \phi^{-1}\circ\phi(x))) = \alpha_Y(g, \phi(x)).
    \]
\end{proof}

We can now state a lemma telling us that if a composite function is equivariant, then it must be a composite of equivariant functions.

\begin{lemma}
    Assume that we are given a group $G$ and two sets $X$ and $Z$ with group actions
    $\alpha_X$ and $\alpha_Z$.
    Assume also that we are given a further set $Y$ and two functions
    $\phi: X\to Y$ and $\psi: Y\to Z$ such that their
    composition $\psi\circ\phi: X\to Z$ is $G$-equivariant w.r.t. $\alpha_X$ and $\alpha_Z$.
    \begin{enumerate}
    \item If $\psi$ is invertible we can define a group action $\alpha_Y$ on $Y$
    such that $\phi$ and $\psi$ are $G$-equivariant with respect to this action.
    \item If $\psi$ is not invertible we can in a natural way modify $Y$ to a space $Y'$ and define a group action $\alpha_{Y'}$ on $Y'$ such that
    $\phi$ and $\psi$ are equivariant when seen as functions to/from $Y'$.
    \end{enumerate}
\end{lemma}
\begin{proof}
Assume first that $\psi$ is invertible.
Define $\alpha_Y:G\times Y\to Y$ by 
\[
    \alpha_Y(g, y) = \psi^{-1}(\alpha_Z(g, \psi(y))).
\]
We need to show that this defines a group action.
For the identity element $i\in G$ we have
\[
    \alpha_Y(i, y) = \psi^{-1}(\alpha_Z(i, \psi(y))) = \psi^{-1}(\psi(y)) = y.
\]
Secondly, for $g, h\in G$ and $y\in Y$ arbitrary we have
\[
\begin{split}
    \alpha_Y(hg, y) &= \psi^{-1}(\alpha_Z(hg, \psi(y))) \\
    &= \psi^{-1}(\alpha_Z(h, \alpha_Z(g, \psi(y))) \\
    &= \psi^{-1}(\alpha_Z(h, \psi(\alpha_Y(g, y)))) \\
    &= \psi^{-1}(\psi(\alpha_Y(h, \alpha_Y(g, y)))) \\
    &= \alpha_Y(h, \alpha_Y(g, y)).
\end{split}
\]
Thus $\alpha_Y$ is a group action.

We note directly that $\psi$ is equivariant as
\[
\alpha_Z(g, \psi(y)) = \psi(\alpha_Y(g, y))
\]
by definition of $\alpha_Y$.
Next we show that $\phi$ is equivariant, which follows from the fact
that $\psi\circ\phi$ is equivariant:
\[
\begin{split}
    \alpha_Y(g, \phi(x)) &= \psi^{-1}(\alpha_Z(g, \psi\circ\phi(x))) \\
    &= \psi^{-1}(\psi\circ\phi(\alpha_X(g, x))) \\
    &= \phi(\alpha_X(g, x)).
\end{split}
\]

If $\psi$ is not invertible, then we can introduce $Y'=\phi(X)/\sim$
where $\sim$ is the equivalence relation identifying elements of $Y$ that map to the same element of $Z$, i.e. 
\[
y_1\sim y_2 :\Longleftrightarrow \psi(y_1) = \psi(y_2).
\]
Then $\psi$ is invertible as a map $\psi: Y'\to\psi\circ\phi(X)$.
Note that the action $\alpha_Z$ is well defined even when restricting from $Z$ to $\psi\circ\phi(X)$,
because by the equivariance of $\psi\circ\phi$,
$\alpha_Z$ can't move an element
from $\psi\circ\phi(X)$ to $Z\setminus\psi\circ\phi(X)$:
\[
\alpha_Z(g, \psi\circ\phi(x)) = \psi\circ\phi(\alpha_X(g, x))\in \psi\circ\phi(X).
\]
Hence the earlier argument for constructing $\alpha_Y$ works for
constructing a group action $\alpha_{Y'}$ on $Y'$ such that the maps $\phi$ and $\psi$ (appropriately restricted) become equivariant.
\georg[inline]{Det känns som att det borde vara möjligt att utöka $\alpha_{Y'}$ till ett $\alpha_{Y}$ och att skriva det här lemmat lite snyggare. PROBLEM: $\phi$ kanske inte är linjär längre även om den var det från början.}
\end{proof}

\begin{definition}
    Given a group $G$ and a vector space $U$,
    a group action $\alpha: G\times U\to U$ is called a
    \emph{linear group action} or a \emph{representation} of $G$
    if $\alpha$ is linear in the second argument.
\end{definition}

\begin{lemma}
    If $\phi$ is a linear map between the vector spaces $U$ and $V$,
    and there is a linear group action $\alpha_U$ on $U$ and an
    arbitrary group action $\alpha_V$ on $V$ such that $\phi$ is equivariant with respect to these, then $\alpha_V$ has to be linear on the image of $\phi$.
\end{lemma}
\begin{proof}
    Take $g\in G$, $x,y\in U$ and $a, b\in\R$ arbitrary.
    We have
    \[
    \begin{split}
        \alpha_V(g, a\phi(x) + b\phi(y)) &= \alpha_V(g, \phi(ax + by)) \\
        &= \phi(\alpha_U(g, ax + by)) \\
        &= a\phi(\alpha_U(g, x)) + b\phi(\alpha_U(g, y)) \\
        &= a\alpha_V(g, \phi(x)) + b\alpha_V(g, \phi(y)).
    \end{split}
    \]
\end{proof}

\begin{lemma}
    Assume that we have a linear group action $\alpha_1$ on the
    vector space $\R^m$ and a second arbitrary group action
    $\alpha_2$ on the same vector space $\R^m$.
    Assume further that the pointwise applied $\ReLU$ activation
    function is equivariant with respect to these actions, i.e. for all $g\in G$, $x\in\R^m$:
    \[
        \ReLU(\alpha_1(g, x)) = \alpha_2(g, \ReLU(x)).
    \]
    Then $\alpha_2$ equals $\alpha_1$ on the image of $\ReLU$.
\end{lemma}
\begin{proof}
    The image of $\ReLU$ is $\R^m_{\geq 0}$. For $x\in\R^m_{\geq 0}$ we have
    \[
        \alpha_2(g, x) = \alpha_2(g, \ReLU(x)) = \ReLU(\alpha_1(g, x)).
    \]
    So if we can show that $\alpha_1(g, x)$ is in $\R^m_{\geq 0}$ we have completed the proof,
    because then $\ReLU(\alpha_1(g, x))=\alpha_1(g, x)$.
    

    
    Thus we now proceed to show that $\alpha_1(g,\cdot)$ maps $\R^m_{\geq 0}$ to itself.
    Take $x\in\R_{\leq 0}^m$ arbitrary (note $\R_{\leq 0}$ rather than $\R_{\geq 0}$).
    We have
    \[
        \ReLU(\alpha_1(g, x)) = \alpha_2(g, \ReLU(x)) = \alpha_2(g, 0)
    \]
    so $\ReLU(\alpha_1(g, x))$ is the same for all $x\in\R_{\leq 0}^m$.
    This means that the positive entries of $\alpha_1(g, x)$ must be the
    same for all $x\in\R_{\leq 0}^m$.
    However, since the negative standard unit basis vectors 
    $-e_i$ lie in $\R_{\leq 0}^m$ and $\alpha_1(g, \cdot)$ is an invertible linear map 
    (with inverse $\alpha_1(g^{-1}, \cdot)$),
    the images under $\alpha_1(g, \cdot)$ of the $-e_i$'s must span $\R^m$.
    Hence the images $-\alpha_1(g, e_i)$ can not have a shared constant
    entry and since any positive entry would have to be equal for
    all images by the above argument, we conclude that 
    $-\alpha_1(g, e_i)\in\R_{\leq 0}^m$.
    From this we get immediately that $\alpha_1(g, e_i)\in\R_{\geq 0}^m$
    so that $\alpha_1(g, \cdot)$ maps $\R_{\geq 0}^m$ to itself.
    

\end{proof}

